On-The-Fly Static Analysis via Dynamic Bidirected Dyck Reachability

Dyck reachability is a principled, graph-based formulation of a plethora of static analyses. Bidirected graphs are used for capturing dataflow through mutable heap data, and are usual formalisms of demand-driven points-to and alias analyses. The best (offline) algorithm runs in $O(m+n\cdot \alpha(n))$ time, where $n$ is the number of nodes and $m$ is the number of edges in the flow graph, which becomes $O(n^2)$ in the worst case. In the everyday practice of program analysis, the analyzed code is subject to continuous change, with source code being added and removed. On-the-fly static analysis under such continuous updates gives rise to dynamic Dyck reachability, where reachability queries run on a dynamically changing graph, following program updates. Naturally, executing the offline algorithm in this online setting is inadequate, as the time required to process a single update is prohibitively large. In this work we develop a novel dynamic algorithm for bidirected Dyck reachability that has $O(n\cdot \alpha(n))$ worst-case performance per update, thus beating the $O(n^2)$ bound, and is also optimal in certain settings. We also implement our algorithm and evaluate its performance on on-the-fly data-dependence and alias analyses, and compare it with two best known alternatives, namely (i) the optimal offline algorithm, and (ii) a fully dynamic Datalog solver. Our experiments show that our dynamic algorithm is consistently, and by far, the top performing algorithm, exhibiting speedups in the order of 1000X. The running time of each update is almost always unnoticeable to the human eye, making it ideal for the on-the-fly analysis setting.

==> algorithms/fixpoint.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
\caption{$\DynamicFixpoint()$}\label{algo:dynamic_fixpoint}
\BlankLine
\While(\tcp*[f]{Repeat until fixpoint}){$\Queue$ is not empty}{\label{line:fixpoint_loop_outer}
Extract $(u, \CloseParenthesis)$ from $\Queue$\label{line:fixpoint_extract}\tcp*[f]{We will merge components connected via $u$'s component}\\
\uIf(\tcp*[f]{$u$ is the root of its component}){$u=\DisjointSets.\Find(u)$}{\label{line:fixpoint_if_parent}
$S\gets \{\DisjointSets.\Find(w):w\in \Edges[u][\CloseParenthesis]\}$\label{line:fixpoint_construct_s}\tcp*[f]{The components to be merged}\\
\eIf{$|S|\geq 2$}{\label{line:fixpoint_if_two}
\textcolor{black}{Insert $\CloseParenthesis$ in $\ActiveLabels[u]$}\tcp*[f]{Record that $\DSCC(u)$ has merged components using $\CloseParenthesis$}\\
$x\gets $ some arbitrary element of $S\setminus\{u\}$\label{line:fixpoint_choose_x}\tcp*[f]{$x$ will be the root of the merged component}
\textcolor{black}{\\
\ForEach(\tcp*[f]{$y$ is no longer the root of its component, as it was merged}){$y\in S\setminus \{ x\}$}{
Insert all $\ActiveLabels[y]$ in $\ActiveLabels[x]$\tcp*[f]{As $x$ is the root of the new component}\\
$\ActiveLabels[y]\gets \emptyset$
}
}
Make $\DisjointSets.\Union(S,x)$\label{line:fixpoint_update_scc}\tcp*[f]{All components merge to $x$'s component}\\
\ForEach(\tcp*[f]{Process each label separately}){label $\CloseParenthesisBeta\in\SetClosedParenthesis$}{\label{line:fixpoint_loop_append}
\ForEach{$v\in S\setminus\{x\}$}{\label{line:fixpoint_loop_inner}
\eIf(\tcp*[f]{$(v, \CloseParenthesisBeta)$ is not the $(u, \CloseParenthesis)$ we extracted from $\Queue$}){$u\neq v$ or $i\neq j$}{\label{line:fixpoint_if_move}
Append $\Edges[v][\CloseParenthesisBeta]$ to $\Edges[x][\CloseParenthesisBeta]$\label{line:fixpoint_append}\tcp*[f]{In $O(1)$ time, using pointers}\\
}
{
Append $(x)$ to $\Edges[x][\CloseParenthesisBeta]$\label{line:fixpoint_append2}\tcp*[f]{All $\Edges[u][\CloseParenthesis]$ merged to a self-loop $x\DTo{\CloseParenthesis}x$}
}
}
\lIf(\tcp*[f]{More components to be merged}){$|\Edges[x][\CloseParenthesisBeta]|\geq 2$}{
Insert $(x, \CloseParenthesisBeta)$ in $\Queue$\label{line:fixpoint_queue_insert2}
}
}
}
{
Let $x\gets$ the single node in $S$
}
\lIf{$u\not \in S$ or $|S|=1$}{\label{line:fixpoint_if_update}
$\Edges[u][\CloseParenthesis]\gets (x)$\label{line:fixpoint_new_edges}\tcp*[f]{$u$'s component now points to $x$'s component}
}
}
}
\end{algorithm}

==> algorithms/makeprimary_bk.tex <==
\smallskip
\begin{algorithm}%[H]
\small
\DontPrintSemicolon
\caption{$\MakePrimary()$}\label{algo:make_primary}
\BlankLine
%\lIf(\tcp*[f]{$u\DTo{\CloseParenthesis}v$ has not merged in $\DSCC(v)$}){$\CloseParenthesis\not\in \ActiveLabels[\DisjointSets.\Find(u)]$}{
%\Return{}
%}
\tcp{1. A forward search from $\DSCC(u)$ to gather the DSCCs potentially affected by the delete}
$\Stack\gets$ an empty queue over $V\times \SetClosedParenthesis$\tcp*[f]{A simple queue to perform the forward search}\\
$\AffectedDSCCs\gets$ an empty set over $V$\tcp*[f]{Stores the roots of DSCCs potentially affected by the delete}\\
Insert $(\DisjointSets.\Find(v), \CloseParenthesis)$ in $\Stack$\tcp*[f]{Start the forward search from $\DSCC(u)$}\\
\While{$\Stack$ is not empty}{
Extract $(x, \CloseParenthesisBeta)$ from $\Stack$\\
$y\gets$ the unique node in $\Edges[\DisjointSets.\Find(x)][\CloseParenthesisBeta]$\tcp*[f]{Unique due to component merging}\\
$z\gets \DisjointSets.\Find(y)$\tcp*[f]{The root of $\DSCC(y)$}\\
\uIf(\tcp*[f]{This is the first time we encounter $\DSCC(z)$}){$z\not \in \AffectedDSCCs$}{
Insert $z$ in $\AffectedDSCCs$\tcp*[f]{Mark $\DSCC(z)$ as potentially affected by the delete}\\
\ForEach(\tcp*[f]{The labels $\DSCC(z)$ might used to merge neighbor DSCCs}){$\CloseParenthesisGamma\in \ActiveLabels[z]$}{
Insert $(z, \CloseParenthesisGamma)$ in $\Stack$\tcp*[f]{Mark for further processing}\\
}
}
}
\tcp{2. Every DSCC potentially affected is split to its PDSCCs}
$\NewRoots\gets$ an empty set over $V$\\
\ForEach{$z\in \AffectedDSCCs$}{
Split the nodes of $z$'s component in $\DisjointSets$ to its PDSCCs, using $\PrimCompDS$\\
Insert the roots of the new components in $\NewRoots$
}
\tcp{3. Gather edges incoming to the newly initialized components for new fixpoint computation}
%Remove $\CloseParenthesis$ from $\ActiveLabels[\DisjointSets.\Find(u)]$\tcp*[f]{$\CloseParenthesis$ might no longer be active in $u$'s DSCC}\\
$\NewIncomingRoots\gets$ an empty set over $V\times \SetClosedParenthesis$\\
\ForEach(\tcp*[f]{Iterate over the roots of the newly split components}){$r\in \NewRoots$}{
\ForEach(\tcp*[f]{Iterate over the nodes of each newly split component}){$s$ in the component of $r$}{
\ForEach{label $\CloseParenthesisBeta\in\SetClosedParenthesis$}{
\ForEach(\tcp*[f]{Retrieve that $t\DTo{\CloseParenthesisBeta}\PDSCC(s)$}){$t\in \InEdges[s][\CloseParenthesisBeta]$}{
$x\gets \DisjointSets.\Find(t)$\tcp*[f]{The root of $r$'s component}\\
%\uIf(\tcp*[f]{Edges $t\DTo{\CloseParenthesisBeta}\cdot$ potentially formed a PDSCC}){$|\OutEdges[t][\CloseParenthesisBeta]|\geq 2$}{
%Insert $\CloseParenthesisBeta$ in $\ActiveLabels[x]$\tcp*[f]{So $\CloseParenthesisBeta$ is potentially an active label of $t$'s DSCC}\\
%}
Insert $s$ in $\Edges[x][\CloseParenthesisBeta]$\tcp*[f]{The component of $t$ has an outgoing edge to $s$}\\
Insert $(x, \CloseParenthesisBeta)$ in $\NewIncomingRoots$\tcp*[f]{Mark that we have inserted edges in $\Edges[x][\CloseParenthesisBeta]$}\\
}
}
}
}
\ForEach(\tcp*[f]{Re-initialize the queue $\Queue$ for the new fixpoint}){$(x,\CloseParenthesisBeta)\in \NewIncomingRoots$}{
\uIf(\tcp*[f]{There are two outgoing  $\CloseParenthesisBeta$-labeled edges from $x$'s component}){$|\Edges[x][\CloseParenthesisBeta]|\geq 2$}{
Insert $(x, \CloseParenthesisBeta)$ in $\Queue$\\
}
}
\end{algorithm}

==> app_example.tex <==
\section{Example}\label{sec:app_example}
In this section we give a step-by-step illustration of $\DynamicAlgo$ on the example of \cref{fig:illustrative_example}.
The components in the $\DisjointSets$ and $\PrimCompDS$ data structures are listed as sequences of nodes $[(a),b,c,\dots]$, where the node in the parenthesis denotes the representative of the component.

\Paragraph{Data Structures before the highlighted changes}
We start with a description of the contents of the various data structures before handling the edge insertion.
\begin{compactenum}
    \item $\Count : [(c,g,\ov{R}\colon 1) , (f,c,\ov{L}\colon 1) , (f,e,\ov{L}\colon 1) , (f,d,\ov{L}\colon 1) , (g,e,\ov{L}\colon1) , (h,f,\ov{L}\colon 1)]$
    \item $\OutEdges: [f,\ov{L}\colon (e,c,d)] , [g,\ov{L}\colon (e)] , [h,\ov{L}\colon (f)], [c,\ov{R}\colon (g)]$
    \item $\InEdges: [d,\ov{L}\colon (f)], [e,\ov{L}\colon (g)], [f,\ov{L}\colon (h)], [g,\ov{R}\colon (c)]$
    \item $\Edges: [(f,\ov{L}): (c)] , [(c,\ov{R}): (g)], [(g,\ov{L}): (e)], [(h,\ov{L}): (f)]$
    \item $\DisjointSets: [(c),d,e], [(g)], [(f)], [(h)]$
    \item $\PrimCompDS-\PDSCC: [(c),d,e], [(g)], [(f)], [(h)]$
    \item  $\Queue : \emptyset$
\end{compactenum}
\Paragraph{After inserting edge $(d,h,\ov{R})$.}
We now describe the development of the data structures during the edge insertion.
\begin{compactenum}
    \item $\Count[d][h][\ov{R}] = 1$.
    \item Since $|\OutEdges[d][\ov{R}]| == 0$, the algorithm adds $d$ to the $\InEdges[h][\ov{R}]$, i.e $\InEdges[h][\ov{R}] = (d)$.
    Then, the  algorithm inserts $h$ as the head of $\OutEdges[d][\ov{R}]$. So, $\OutEdges[d][\ov{R}] = (h)$. 
    \item Get the root of $\DSCC$ containing $d$ , i.e. $c = \DisjointSets.\Find(d)$. 
    Then add $h$ to $\Edges[c][\ov{R}]$. 
    So, updated $\Edges[c][\ov{R}] = (g,h)$. 
    \item Since, $|\Edges[c][\ov{R}]| \ge 2$. 
    The algorithm inserts $(c,\ov{R})$ in $\Queue$ and invokes $\Fixpoint()$.
    \item Inside $\Fixpoint()$: First, we extract $(c,\ov{R})$ from $\Queue$. 
    Then we get the set $S = \{g,h\}$. 
    Since $|S| \ge 2$, the algorithm merges  $\DSCC$s $[(g)], [(h)]$ into single $\DSCC [(h),g]$. 
    Then, moves $\Edges[g][\ov{L}]$ to $\Edges[h][\ov{L}]$.
    Now, since $|\Edges[h][\ov{L}]| \ge 2$, insert $(h,\ov{L})$ to $\Queue$.
    This will lead to merging of $\DSCC$s $[(c),d,e]$ and $[(f)]$ into $\DSCC$ $[(f),c,d,e]$.
    This finishes the fixpoint.
\end{compactenum}

After the insertion, the data structures are in the following state.

\begin{compactenum}
    \item $\Count$:- new entry $(d,h,\ov{R}\colon 1)$
    \item $\OutEdges$:- new entry $[d,\ov{R}\colon (h)]$
    \item $\InEdges$: new entry $[h,\ov{R}\colon (d)]$
    \item $\Edges: [(f,\ov{L}): (c)] , [(f,\ov{R}): (h)], [(h,\ov{L}): (f)]$
    \item $\DisjointSets: [(f),c,d,e], [(h) , g]$
    \item $\PrimCompDS-\PDSCC: [(c),d,e], [(g)], [(f)], [(h)]$
    \item  $\Queue : \emptyset$
\end{compactenum}

\Paragraph{After deleting edge $(f,d,\ov{L})$.}
We now describe the development of the data structures during the edge deletion.
\begin{compactenum}
    \item $\Count[f][d][\ov{L}] = 0$.
    \item Since $d$ is at tail of $\OutEdges[f][\ov{L}]$, remove $f$ from $\InEdges[d][\ov{L}]$.
    \item In $\OutEdges[f][\ov{L}]$, $c$ is penultimate element. 
    Hence, the algorithm inserts $f$ in $\InEdges[c][\ov{L}]$.
    So the updated $\InEdges$ is $\{ [c,\ov{L}\colon (f)], [e,\ov{L}\colon (g)], [f,\ov{L}\colon (h)], [g,\ov{R}\colon (c)], [h,\ov{R}\colon (d)]\}$.
    \item Remove edge $(c,d)$ from $\PrimCompDS$. 
    Hence, the updated $\PrimCompDS-\PDSCC$ 
    will be $\{ [(c),e] , [(d)], [(g)] , [(f)] , [(h)] \}$.  
    \item Remove $d$ from $\OutEdges[f][\ov{L}]$.
    \item Invoke $\MakePrimary()$:
        \begin{compactenum}
            \item 
            % Since there exists node other than $d$ in $\DSCC(d)$ $(e or c)$ such that $\DSCC(f) \DTo{\CloseParenthesis} e$, 
            Insert $f=\DSCCRep(d)$ to $\Stack$ and $\AffectedDSCCs$.
        \item In the loop from \cref{line:algo_makeprimary_fwdsearchloop} to \cref{line:algo_makeprimary_firststepend} in 
        % Algorithm \cref{algo:make_primary}, 
       the  algorithm inserts $h=\DSCCRep(g)$ to $\Stack$ and $\AffectedDSCCs$. 
        \item $\AffectedDSCCs$ contains $f, h$ and by following $\InEdges$, algorithm re-initializes $\Edges[f][\ov{L}]$, $\Edges[f][\ov{R}]$ and $\Edges[h][\ov{L}]$ to an empty list.
        % (\cref{line:unaffected}).
        \item Since $\AffectedDSCCs$ contains $f$ and $h$, we split $\DSCC(f)$ and $\DSCC(h)$ to their $\PDSCC$s. 
        Hence, the updated $\DisjointSets$ is $\{ [(c),e] , [(d)], [(g)] , [(f)] , [(h)] \}$.
        Then the algorithm inserts roots of new components in $\NewRoots$. 
        So, we get $\NewRoots = \{ c , d , f, g, h\}$.
        % For each edgetype $\CloseParenthesisBeta$ algorithm reinitialize $\Edges[f][\CloseParenthesisBeta]$ and $\Edges[h][\CloseParenthesisBeta]$.
        \item In the next step the algorithm gathers edges for fixpoint computations. 
        For each root $r$ in $\NewRoots$, the algorithm iterate over all nodes in $\DSCC(r)$.
        For each node $t$ in $\DSCC(r)$ and each edge type $\CloseParenthesisBeta \in \{\ov{L} , \ov{R}\}$ the algorithm checks if there exists node $s \in \InEdges[t][\CloseParenthesisBeta]$.
        For all such nodes $s$, the algorithm inserts $t$ in $\Edges[\DSCCRep(s)][\CloseParenthesisBeta]$ 
        and $(\DSCCRep(s),\CloseParenthesisBeta)$ in $\NewIncomingRoots$ (lines \cref{line:algo_makeprimary_iterateoverpdsccinedges} to \cref{line:populate_L}) .
        In lines \cref{line:algo_makeprimary_edgelist_of_pdsccs} - \cref{line:algo_makeprimary_insert_y_in_edges_r} the algorithm checks if $\OutEdges[t][\CloseParenthesisBeta] \ge 1$. 
        If yes, then inserts $x=$ first node of $\OutEdges[t][\CloseParenthesisBeta]$ in $\Edges[r][\CloseParenthesisBeta]$.

        So after \cref{line:algo_makeprimary_insert_y_in_edges_r} the updated $\Edges$ data structures will be 
        $\{ [(c,\ov{R}):(g)] , [(f,\ov{L}):(c)], [(h,\ov{L}):(f)] [(g,\ov{L}):(e)], [(d,\ov{R}):(h)] \}$. 
        And $\NewIncomingRoots$ will contain $\{ (d,\ov{R}), (f,\ov{L}), (c,\ov{R}) , (g,\ov{L}), (h,\ov{L}) \}$.
        \item
        Then the algorithm iterates over all $(x,\CloseParenthesisBeta)$ $ \in \NewIncomingRoots$,
        and checks if $\Edges[x][\CloseParenthesisBeta] \ge 2$. 
        If yes, then inserts $(x,\CloseParenthesisBeta)$ in $\Queue$.  
        So, for $\NewIncomingRoots = \{ (d,\ov{R}), (f,\ov{L}), (c,\ov{R}) , (g,\ov{L}), (h,\ov{L}) \}$ 
        no element will be added to the $\Queue$.
        \end{compactenum}

        \item Since $\Queue$ is empty, the call to $\Fixpoint()$ will not merge any components.
\end{compactenum}
Hence, the $\DSCC$s after delete are $\{ [(c),e] , [(d)], [(g)] , [(f)] , [(h)] \}$.

After the deletion, the data structures are in the following state.
\begin{compactenum}
   \item $\Count : [(c,g,\ov{R}\colon 1) , (f,c,\ov{L}\colon 1) , (f,e,\ov{L}\colon 1) , (f,d,\ov{L}\colon 0) , (g,e,\ov{L}\colon1) , (h,f,\ov{L}\colon 1) , (d,h,\ov{R}\colon 1)]$
    \item $\OutEdges: [f,\ov{L}\colon (e,c)] , [g,\ov{L}\colon (e)] , [h,\ov{L}\colon (f)], [c,\ov{R}\colon (g)] , [d,\ov{R}\colon (h)]$
    \item $\InEdges: [c,\ov{L}\colon (f)], [e,\ov{L}\colon (g)], [f,\ov{L}\colon (h)], [g,\ov{R}\colon (c)] , [h,\ov{R}\colon (d)]$
    \item $\Edges: [(c,\ov{R}):(g)] , [(f,\ov{L}):(c)], [(h,\ov{L}):(f)] [(g,\ov{L}):(e)], [(d,\ov{R}):(h)] $
    \item $\DisjointSets: [(c),e] , [(d)], [(g)] , [(f)] , [(h)]$
    \item $\PrimCompDS-\PDSCC: [(c),e] , [(d)], [(g)] , [(f)] , [(h)]]$
    \item  $\Queue : \emptyset$
\end{compactenum}


==> app_mistakes_in_earlier_approaches.tex <==
\section{Mistakes in earlier approaches}\label{sec:app_mistakes_in_earlier_approaches}

As a sanity check, here we plot the quadratic runtime behavior that the tool accompanying~\cite{Li2022} has on the counterexamples of \cref{fig:mistake_complexity_graphs} from \cref{sec:mistakes}.

\input{figures/mistake_complexity_plots}

%We will explain the error in Procedure 4 of \cite{Li2022} using the example in \cref{fig:mistake_correctness}.
%Assuming we represent the graph with opening paranthesis to be consistent with Procedure 4 of \cite{Li2022}.
%We will be ignoring paranthesis type for simplicity, since in the current example all paranthesis types are same.
%
%Delete in edge $(x2,u)$ causes procedure SplitFurther() to be called on merged graph nodes $\{u\}$ and $\{x1,x2\}$. 
%
%$SplitFurther(u,G,Gm)$ returns from line 8, since there are no outgoing edges from u and merged node $\{u\}$ contains single node.
%
%$SplitFurther(\{x1,x2\},G,Gm)$ is explained as follows:
%\begin{compactenum}
%\item Line 3 : groups = $\{\{x1\}, \{x2\}\}$
%\item Line 4 : outgoing edges from $\{x1,x2\}$ with weight > 1 : [ $\{x1,x2\}$ -> $\{u\}$ , $\{x1,x2\}$ -> $\{y1,y2\}$ ]
%\begin{compactenum}
%\item For e' = $\{x1,x2\}$ -> $\{u\}$:
%\begin{compactenum}
%\item Edges merged into e' = [x1 -> u]
%\item $s_i = \{x1\}$
%\end{compactenum} 
%\item For e' = $\{x1,x2\}$ -> $\{y1,y2\}$:
%\begin{compactenum}
%\item Edges merged into e' = [x1 -> y1, x2 -> y2]
%\item $s_i = \{x1,x2\}$
%\end{compactenum} 
%\end{compactenum} 
%
%\item Line 6 : merges $s_i$ in merged graph : groups = $\{\{x1,x2\}\}$
%
%\item Line 7 : Size(groups) = Size( $\{\{x1,x2\}\}$ ) = 1, therefore return with no split in merged node $\{x1,x2\}$.
%
%\end{compactenum}
%
%Therefore, Procedure 4 of \cite{Li2022} keeps $\{x1,x2\}$ merged as it incorrectly assumes a dyck path via $\{y1,y2\}$.
%
%\input{counterexample_complexity_plots}

==> counterexample_complexity_plots.tex <==
\begin{figure}
\pgfplotsset{every tick label/.append style={font=\small}}
\def\plotwidth{7cm}
\def\offlinecolor{black!20}
\def\dynamiccolor{black!60}
\scalebox{0.9}{%
\begin{subfigure}[b]{0.475\textwidth}
\begin{tikzpicture}
\begin{axis}[
    %title={Running time on $\DeleteEdge(u,b_1,\CloseParenthesis)$ vs $n$},
    xlabel={$n$},
    ylabel={milliseconds},
    xmin=0, xmax=1700,
    % ymin=0, ymax=01,
    % ytick={0,0.2,0.4,0.6,0.8,1},
    %xtick={0,200,400,600,800,1000,1200,1400,1600},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=\plotwidth,
    legend style={font=\small},
    ylabel near ticks,
    xlabel near ticks,
    legend cell align={left},
]

\addplot [color=blue,mark=*] file {figures/dense_offline.dat};
\addplot[color=red,mark=square*] file {figures/dense_dyn.dat};
\legend{Offline,Dynamic}

\end{axis}
\end{tikzpicture}
\caption{
Dense inputs.
\label{subfig:complexity_plots_dense}
}
\end{subfigure}
}
\hfill
\scalebox{0.9}{%
\begin{subfigure}[b]{0.475\textwidth}
\begin{tikzpicture}
\begin{axis}[
   % title={Running time on $\DeleteEdge(u,c_1,\CloseParenthesis)$ vs $n$},
    xlabel={$n$},
    ylabel={milliseconds},
    xmin=0, xmax=1300,
    % ymin=0, ymax=0.09,
    % ytick={0,0.02,0.04,0.06,0.08},
    yticklabel style={/pgf/number format/fixed},
    %xtick={0,500,1000,1300},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    width=\plotwidth,
    legend style={font=\small},
    ylabel near ticks,
    xlabel near ticks,    
    legend cell align={left},
]

\addplot[color=blue,mark=*] file {figures/sparse_offline.dat};
\addplot[color=red,mark=square*] file {figures/sparse_dyn.dat};

\legend{Offline,Dynamic}
\end{axis}
\end{tikzpicture}
\caption{
Sparse inputs.
\label{subfig:complexity_plots_sparse}
}
\end{subfigure}
}
\caption{
Running time of the offline and dynamic algorithms on the dense graphs of \cref{subfig:complexity_plots_dense} (\protect\subref{subfig:complexity_plots_dense}) and sparse graphs of \cref{subfig:complexity_plots_sparse} (\protect\subref{subfig:complexity_plots_sparse}).
\label{fig:complexity_plots}
}
\end{figure}

==> experiments_alias.tex <==
\subsection{Experiments on Alias Analysis}\label{subsec:experiments_alias}

\Paragraph{Formulation of alias analysis.}

%\input{figures/expt_alias_graphs}
%input{figures/expt_alias_ddlog_graphs}

The plot in \cref{fig:expt_alias_graphs} shows the running time of proposed algorithm and offline algorithm over the DaCapo benchmarks \cite{DaCapo:paper} \cite{DaCapo:TR}. The input graphs (initial graph and sequence of operations) for the same are synthesized and provided by \cite{Li2022} in their artifact submission.
The plot in \cref{fig:expt_alias_ddlog_graphs} shows the running time of the proposed algorithm compared to its differential datalog implementation over the DaCapo benchmarks for alias analysis.

==> experiments_data_dependence.tex <==
\subsection{Experiments on Data-Dependence Analysis}\label{subsec:experiments_data_dependence}

\Paragraph{Formulation of data-dependence analysis.}

%\input{figures/expt_datadep_graphs}
%\input{figures/expt_datadep_ddlog_graphs}

The plot in \cref{fig:expt_datadep_graphs} shows the running time of proposed algorithm and offline algorithm over the Data Dependence analysis. The input graphs (initial graph and sequence of operations) for the same are synthesized and provided by \cite{Li2022} in their artifact submission.
The plot in \cref{fig:expt_datadep_ddlog_graphs} shows the running time of the proposed algorithm compared to its differential datalog implementation over the Data Dependence analysis.

==> experiments_grouped.tex <==
\begin{figure}
\captionsetup[subfigure]{aboveskip=-1pt,belowskip=-1pt}

\pgfplotsset{very tick label/.append style={font=\small}}
\def\RatioDataDependence{.58}
\def\PlotWidthDataDependence{9cm}
\def\PlotWidthAlias{6.5cm}
\def\RatioAlias{.38}
%\def\PlotWidth{15cm}

\def\subfigureTextWidthDataDependence{\NumBenchmarksDataDependence/\NumBenchmarksTotal}
\def\subfigureTextWidthAlias{\NumBenchmarksAlias/\NumBenchmarksTotal}

\def\plotheight{4cm}
\def\barwidth{2.5pt}
\def\bardistance{1pt}
\def\scaleboxvalue{0.9}

\def\offlinecolor{black!10}
\def\ddLogcolor{black!50}
\def\dynamiccolor{black!80}


\begin{subfigure}[T]{\RatioDataDependence\textwidth}
\scalebox{\scaleboxvalue}{%
\begin{tikzpicture}[tight background, inner sep=2pt,]
\begin{axis}[inner sep=2pt,
		title={\large \underline{Data Dependence Analysis}},
    ybar=\bardistance,
		enlarge y limits={abs=0.6cm,upper},
		enlarge x limits={abs=8pt},
		legend style={legend pos=north west, draw=black, legend columns=-1,/tikz/every even column/.append style={column sep=0.2cm}},
		ylabel near ticks,
    ylabel={microsecs},
		xtick pos=left,
    xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
    xticklabels={btree,check,compiler,compress,crypto,derby,helloworld,mpegaudio,mushroom,parser,sample,scimark,startup,sunflow,xml},
    ymajorgrids=true,
    grid style=dashed,
    %width=\RatioDataDependence*\PlotWidth,
		width=\PlotWidthDataDependence,
		height=\plotheight,
    legend style={font=\footnotesize},
    xticklabel style={font=\footnotesize,rotate=45,anchor=east},
    yticklabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    bar width=\barwidth,
    ymode=log,
    log origin=infty,
]

\addplot [fill=\offlinecolor] file {figures/expt_datadep_offline_incr.dat};
\addplot [fill=\ddLogcolor] file {figures/expt_datadep_dyn_incr_ddlog.dat};
\addplot[fill=\dynamiccolor] file {figures/expt_datadep_dyndyck_incr.dat};
\legend{Offline,DDlog,Dynamic}

\end{axis}
\end{tikzpicture}
}%
\caption{\label{subfig:datadependence_all_incr}
Incremental updates.
}
\end{subfigure}
\hspace*{\fill}
\begin{subfigure}[T]{\RatioAlias\textwidth}
\scalebox{\scaleboxvalue}{%
\begin{tikzpicture}[tight background]
\begin{axis}[inner sep=2pt,,
		title={\large \underline{Alias Analysis}},
    ybar=\bardistance,
		enlarge y limits={abs=0.6cm,upper},
		enlarge x limits={abs=8pt},
		legend style={legend pos=north west, draw=black, legend columns=-1,/tikz/every even column/.append style={column sep=0.2cm}},
		ylabel near ticks,
    ylabel={microsecs},
		xtick pos=left,
    xtick={1,2,3,4,5,6,7,8,9,10,11},
    xticklabels={antlr, bloat, chart, eclipse, fop, hsqldb, jython, luindex, lusearch, pmd, xalan},
    ymajorgrids=true,
    grid style=dashed,
    %width=\RatioAlias*\PlotWidth,
		width=\PlotWidthAlias,
		height=\plotheight,
    legend style={font=\footnotesize},
    xticklabel style={font=\footnotesize,rotate=45,anchor=east},
    yticklabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    bar width=\barwidth,
    ymode=log,
    log origin=infty,
]

\addplot [fill=\offlinecolor] file {figures/expt_alias_offline_incr.dat};
\addplot [fill=\ddLogcolor] file {figures/expt_alias_dyn_incr_ddlog.dat};
\addplot[fill=\dynamiccolor] file {figures/expt_alias_dyndyck_incr.dat};
\legend{Offline,DDlog,Dynamic}

\end{axis}
\end{tikzpicture}
}%
\vspace{7pt}
\caption{\label{subfig:alias_all_incr}
Incremental updates.
}
\end{subfigure}
\\[1em]
\begin{subfigure}[T]{\RatioDataDependence\textwidth}
\scalebox{\scaleboxvalue}{%
\begin{tikzpicture}[tight background, inner sep=2pt,]
\begin{axis}[inner sep=2pt,
		%title={\large Data Dependence Analysis},
    ybar=\bardistance,
		enlarge y limits={abs=0.6cm,upper},
		enlarge x limits={abs=8pt},
		legend style={legend pos=north west, draw=black, legend columns=-1,/tikz/every even column/.append style={column sep=0.2cm}},
		ylabel near ticks,
    ylabel={microsecs},
		xtick pos=left,
    xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
    xticklabels={btree,check,compiler,compress,crypto,derby,helloworld,mpegaudio,mushroom,parser,sample,scimark,startup,sunflow,xml},
    ymajorgrids=true,
    grid style=dashed,
    %width=\RatioDataDependence*\PlotWidth,
		width=\PlotWidthDataDependence,
		height=\plotheight,
    legend style={font=\footnotesize},
    xticklabel style={font=\footnotesize,rotate=45,anchor=east},
    yticklabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    bar width=\barwidth,
    ymode=log,
    log origin=infty,
]

\addplot [fill=\offlinecolor] file {figures/expt_datadep_offline_decr.dat};
\addplot [fill=\ddLogcolor] file {figures/expt_datadep_dyn_decr_ddlog.dat};
\addplot[fill=\dynamiccolor] file {figures/expt_datadep_dyndyck_decr.dat};
\legend{Offline,DDlog,Dynamic}

\end{axis}
\end{tikzpicture}
}%
\caption{\label{subfig:datadependence_all_decr}
Decremental updates.
}

\end{subfigure}
\hspace*{\fill}
\begin{subfigure}[T]{\RatioAlias\textwidth}
\scalebox{\scaleboxvalue}{%
\begin{tikzpicture}[tight background]
\begin{axis}[inner sep=2pt,,
		%title={\large Alias Analysis},
    ybar=\bardistance,
		enlarge y limits={abs=0.6cm,upper},
		enlarge x limits={abs=8pt},
		legend style={legend pos=north west, draw=black, legend columns=-1,/tikz/every even column/.append style={column sep=0.2cm}},
		ylabel near ticks,
    ylabel={microsecs},
		xtick pos=left,
    xtick={1,2,3,4,5,6,7,8,9,10,11},
    xticklabels={antlr, bloat, chart, eclipse, fop, hsqldb, jython, luindex, lusearch, pmd, xalan},
    ymajorgrids=true,
    grid style=dashed,
    %width=\RatioAlias*\PlotWidth,
		width=\PlotWidthAlias,
		height=\plotheight,
    legend style={font=\footnotesize},
    xticklabel style={font=\footnotesize,rotate=45,anchor=east},
    yticklabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    bar width=\barwidth,
    ymode=log,
    log origin=infty,
]

\addplot [fill=\offlinecolor] file {figures/expt_alias_offline_decr.dat};
\addplot [fill=\ddLogcolor] file {figures/expt_alias_dyn_decr_ddlog.dat};
\addplot[fill=\dynamiccolor] file {figures/expt_alias_dyndyck_decr.dat};
\legend{Offline,DDlog,Dynamic}

\end{axis}
\end{tikzpicture}
}%
\vspace{7pt}
\caption{\label{subfig:alias_all_decr}
Decremental updates.
}
\end{subfigure}
\\[1em]
\begin{subfigure}[T]{\RatioDataDependence\textwidth}
\scalebox{\scaleboxvalue}{%
\begin{tikzpicture}[tight background, inner sep=2pt,]
\begin{axis}[inner sep=2pt,
		%title={\large Data Dependence Analysis},
    ybar=\bardistance,
		enlarge y limits={abs=0.6cm,upper},
		enlarge x limits={abs=8pt},
		legend style={legend pos=north west, draw=black, legend columns=-1,/tikz/every even column/.append style={column sep=0.2cm}},
		ylabel near ticks,
    ylabel={microsecs},
		xtick pos=left,
    xtick={1,2,3,4,5,6,7,8,9,10,11,12,13,14,15},
    xticklabels={btree,check,compiler,compress,crypto,derby,helloworld,mpegaudio,mushroom,parser,sample,scimark,startup,sunflow,xml},
    ymajorgrids=true,
    grid style=dashed,
    %width=\RatioDataDependence*\PlotWidth,
		width=\PlotWidthDataDependence,
		height=\plotheight,
    legend style={font=\footnotesize},
    xticklabel style={font=\footnotesize,rotate=45,anchor=east},
    yticklabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    bar width=\barwidth,
    ymode=log,
    log origin=infty,
]

\addplot [fill=\offlinecolor] file {figures/expt_datadep_offline_mixed.dat};
\addplot [fill=\ddLogcolor] file {figures/expt_datadep_dyn_mixed_ddlog.dat};
\addplot[fill=\dynamiccolor] file {figures/expt_datadep_dyndyck_mixed.dat};
\legend{Offline,DDlog,Dynamic}

\end{axis}
\end{tikzpicture}
}%
\caption{\label{subfig:datadependence_all_mixed}
Mixed updates.
}

\end{subfigure}
\hspace*{\fill}
\begin{subfigure}[T]{\RatioAlias\textwidth}
\scalebox{\scaleboxvalue}{%
\begin{tikzpicture}[tight background]
\begin{axis}[inner sep=2pt,,
		%title={\large Alias Analysis},
    ybar=\bardistance,
		enlarge y limits={abs=0.6cm,upper},
		enlarge x limits={abs=8pt},
		legend style={legend pos=north west, draw=black, legend columns=-1,/tikz/every even column/.append style={column sep=0.2cm}},
		ylabel near ticks,
    ylabel={microsecs},
		xtick pos=left,
    xtick={1,2,3,4,5,6,7,8,9,10,11},
    xticklabels={antlr, bloat, chart, eclipse, fop, hsqldb, jython, luindex, lusearch, pmd, xalan},
    ymajorgrids=true,
    grid style=dashed,
    %width=\RatioAlias*\PlotWidth,
		width=\PlotWidthAlias,
		height=\plotheight,
    legend style={font=\footnotesize},
    xticklabel style={font=\footnotesize,rotate=45,anchor=east},
    yticklabel style={font=\footnotesize},
    ylabel style={font=\footnotesize},
    bar width=\barwidth,
    ymode=log,
    log origin=infty,
]

\addplot [fill=\offlinecolor] file {figures/expt_alias_offline_mixed.dat};
\addplot [fill=\ddLogcolor] file {figures/expt_alias_dyn_mixed_ddlog.dat};
\addplot[fill=\dynamiccolor] file {figures/expt_alias_dyndyck_mixed.dat};
\legend{Offline,DDlog,Dynamic}

\end{axis}
\end{tikzpicture}
}%
\vspace{7pt}
\caption{\label{subfig:alias_all_mixed}
Mixed updates.
}
\end{subfigure}
\caption{\label{fig:experiments}
The average time to handle a single update on on-the-fly data-dependence analysis (\subref{subfig:datadependence_all_incr}, \subref{subfig:datadependence_all_decr}, \subref{subfig:datadependence_all_mixed}) and on-the-fly alias analysis (\subref{subfig:alias_all_incr}, \subref{subfig:alias_all_decr}, \subref{subfig:alias_all_mixed}).
Note that all results are in log-scale.
}
\end{figure}

==> experiments_synthetic.tex <==
\subsection{Experiments on Controlled Graphs}\label{subsec:experiments_synthetic}

\input{figures/expt_controlled_graphs}

The plot in \cref{fig:expt_controlled_graphs} shows the running time of proposed algorithm and offline algorithm over the controlled graphs constructed in \cref{fig:mistake_complexity_graphs}.

==> figures/mistake_graph_dense.tex <==
\begin{figure}
\caption{
\label{fig:mistake_graph1}
}
\end{figure}

==> figures/mistake_graph_sparse.tex <==
\begin{figure}
\caption{
\label{fig:mistake_graph2}
}
\end{figure}

==> figures/mistake_results_dense.tex <==
\begin{figure}
\caption{
\label{fig:mistake_results_dense}
}
\end{figure}

==> figures/mistake_results_sparse.tex <==
\begin{figure}
\caption{
\label{fig:mistake_results_sparse}
}
\end{figure}

==> figures/pdscc_computation.tex <==
\begin{figure}
\caption{
\label{fig:pdscc_computation}
}
\end{figure}
